Learning Continuous Control Policies for Information-Theoretic Active Perception

This paper proposes a method for learning continuous control policies for active landmark localization and exploration using an information-theoretic cost. We consider a mobile robot detecting landmarks within a limited sensing range, and tackle the problem of learning a control policy that maximizes the mutual information between the landmark states and the sensor observations. We employ a Kalman filter to convert the partially observable problem in the landmark state to Markov decision process (MDP), a differentiable field of view to shape the reward, and an attention-based neural network to represent the control policy. The approach is further unified with active volumetric mapping to promote exploration in addition to landmark localization. The performance is demonstrated in several simulated landmark localization tasks in comparison with benchmark methods.

==> tex/Problem.tex <==
\section{Problem Statement}

This section formalizes active exploration and mapping as an optimal control problem. We consider a robot state $\bfx_k \in \R^{n_x}$ and control input $\bfu_k \in \R^m$ at time $t_k \in \R_+$ where $\{t_k\}_{k=0}^K$ for some $K \in \bbN$ is an increasing sequence. The task is to reduce uncertainty in a target state, denoted as $\bfy_k \in \R^{n_y}$, through on-board sensors which receives a sensor measurement.  We consider a deterministic nonlinear dynamics of the system state, a linear stochastic dynamics of the target state described by 
\begin{align}
\bfx_{k+1} &= \bff(\bfx_k, \bfu_k) \label{eq:disc-model}, \\
 \bfy_{k+1} &= A_k \bfy_k + B_k \bfnu_k + \bfw_k , \quad \bfw_k \sim \calN(0, W_k),
\end{align}
where $\bff: \bbR^{n_x} \times \bbR^{n_m} \to \bbR^{n_x}$ is a given function, $\bfnu_k \in \R^{n_{\nu}}$ is an external force term, and $A_k \in \R^{n_y\times n_y}$ and $B_k \in \R^{n_y \times n_{\nu}}$ are given matrices. In the evaluation later, we 
essentially consider a task to 
%consider two scenarios of the target state. One situation is to 
localize a finite number of landmarks $\bfy = [\bfy^{(1)}, \dots, \bfy^{(n_l)}]$, where $\bfy^{(j)}_k \in \R^2$ for $j \in \{1, \dots, n_l\}$ denotes the position of $j$-th landmark and $n_l$ is the total number of landmarks. In additional experiments, we also consider a task of exploring the environment by defining a map state $\bfy_k = \bfm \in \R^{n_m}$ through discretizing $\Omega$ into $h_m \times w_m = n_m \in {\mathbb N}$ tiles, such as voxels or octants \cite{hornung2013octomap}, and associating each tile $j \in {1,\ldots,n}$ with a position $\bfp^{(j)} \in \R^3$ and a mapped value $\bfm^{(j)} \in \R$, such as occupancy or signed distance \cite{oleynikova2017voxblox}. 


To model a limited Field of View (FoV) sensing, we define the set of indices of the landmarks within the field of view $\calF \subset \R^2 $ of the robot, as follows:
%
\begin{align}
    \calI_{k, {\calF}} = \left\{ \forall j \in \{1, \dots, n_l\} \bigg|   \bfq \left(\bfx_k, \bfy^{(j)} \right)  \in \calF \right\}
\end{align}
where $\bfq$ is the robot body-frame coordinates of $\bfy^{(j)}$.
%
Then, the sensor model with limited FoV is formulated as follows:
\begin{align} 
    \bfz_k &= \left[ 
    \begin{array}{c} 
    \{ \bar \bfz(\bfx_k, \bfy^{(j)})\}_{j \in \calI_{k, \calF}}
    \end{array} 
    \right] \in \R^{2 |\calI_{k, \calF}|}, \label{eq:sensor}  \\
  \bar  \bfz(\bfx, \bfy^{(j)}) &=   \bfh (\bfx, \bfy^{(j)} )+ V^{1/2}(\bfx, \bfy^{(j)}) \bfv, \label{eq:slam-sensing} 
\end{align}
where $\Gamma: \R^{n_x} \times \R^2 \to \bbS_{\succ 0}^{2 \times 2}$ is the sensor noise covariance and $\bfv \sim \N (0, I_2)$. 



We formulate active exploration as an optimal control problem over infinite-time horizon, aiming to obtain a control policy $\bfu_k = \bfpi^*(\cdot)$ to minimize the variation of differential entropy\footnote{The differential entropy of a continuous random variable $Y$ with probability density function $p$ is defined as $\bbH(Y) := - \int p(y) \log p(y) dy$.} in the target state: 
\begin{problem*} 
Given a dataset for $\{\bfy_0\}$, obtain a control policy $\bfu_k = \bfpi() $ for given $\bfx_{k}$ and $\bfz_{0:k}$, to solve:
\begin{align} \label{eq:Entropy} 
\bfpi^* &= \argmin_{\bfpi(\cdot)}  \left(  \sum_{k=0}^{\infty} \gamma^{k} \Delta \bbH_k \right),  \\
\Delta \bbH_k &=  \bbH( \bfy_{k+1} | \bfz_{1:k+1}, \bfx_{1:k+1}) - \bbH( \bfy_k | \bfz_{1:k}, \bfx_{1:k}))
\end{align} 
%
subject to the models in \eqref{eq:disc-model}--\eqref{eq:slam-sensing}. 
\end{problem*}



